Speech Intelligibility Assessment of Dysarthric Speech by using Goodness of Pronunciation with Uncertainty Quantification

This paper proposes an improved Goodness of Pronunciation (GoP) that utilizes Uncertainty Quantification (UQ) for automatic speech intelligibility assessment for dysarthric speech. Current GoP methods rely heavily on neural network-driven overconfident predictions, which is unsuitable for assessing dysarthric speech due to its significant acoustic differences from healthy speech. To alleviate the problem, UQ techniques were used on GoP by 1) normalizing the phoneme prediction (entropy, margin, maxlogit, logit-margin) and 2) modifying the scoring function (scaling, prior normalization). As a result, prior-normalized maxlogit GoP achieves the best performance, with a relative increase of 5.66%, 3.91%, and 23.65% compared to the baseline GoP for English, Korean, and Tamil, respectively. Furthermore, phoneme analysis is conducted to identify which phoneme scores significantly correlate with intelligibility scores in each language.

==> figures/_result.tex <==
\begin{table}[t]
\caption{
Kendall's rank coefficient between GoP \& intelligibility severity levels. A higher absolute value indicates a stronger correlation between the two variables.
}
\label{tab:results}
\centering
\resizebox{0.45\textwidth}{!}
{
\begin{tabular}{c|c|c|c|c}
\hline
Experiment & Classifier & English & Korean & Tamil \\
\hline
\multirow{4}{*}{Baselines} 
& GMM-GoP \cite{witt2000phone,hmm-gop} & -0.57 & -0.59 & - \\
& NN-GoP (LPP) \cite{hu2015improved} & -0.49 & -0.65 & -  \\
& ASR free-GoP \cite{Cheng2020ASRFreePA} & -0.58 & -0.70 & - \\
& SSL-GoP \cite{xu2021explore} & &  &\\
% \cline{2-5}
% & ASR-GOP & & &   \\
\hline
\multirow{7}{*}{Proposed} 
& Probability Entropy-GoP & &  &   \\
& Probability Margin-GoP & & &  \\
& Max Logit-GoP & & &   \\
\cline{2-5}
& Normalized Logit-GoP & &  &  \\
& Temperature Scaling-GoP & &  &  \\
& ODIN-GoP & &  &  \\
& Mahalannobis-GoP & & &   \\
\hline
\end{tabular}
}
\vspace{-1em}
\end{table}

% GMM-GOP \cite{hmm-gop} & & &\\
%

==> sections/_2_godness_of_pronunciation.tex <==
\section{Proposed approach} \label{sec:gop}
In this study, seven popular UQ methods are applied to GoP calculations.
Three methods involve modifying the scoring function, and four methods involve modifying the phoneme predictor.
We release the source codes of all the implementations\footnote{\url{https://github.com/juice500ml/dysarthria-gop}}.

\subsection{Prerequisite: Goodness of Pronunciation (GoP)}
In this subsection, we provide a succinct summary of the existing GoP-based methods from the uncertainty quantification perspective.
% understanding the existing GOP literature in the perspective of ood
Given a phone $p$ during frames $f \in F$ with frame-wise phone probability and its logits as $P^f(p|f)$ and $L^f(p|f)$, and the total phone set as $Q$, \textbf{GMM-GOP} \cite{witt2000phone} is defined as follows:
% \subsubsection{GMM-GoP \cite{witt2000phone}}
\begin{equation}
    s_\text{GMM-GoP}(p) = \frac{1}{|F|} \sum_{f \in F} \log \frac{e^{L^f(p|f)}}{ \sum_{q \in Q} e^{L^f(q|f)}},
\end{equation}
which is an averaged log probability across the phone duration, $\mathbb{E}_F[\log P^f(p|f)]$.
Note that directly using the probability output is often used as a baseline for out-of-distribution detection \cite{hendrycks2017baseline}.
Also, averaging acts as a temporal ensembling \cite{laine2017temporal}, where it is often employed also as a baseline for out-of-distribution detection \cite{ovadia2019can}.


\textbf{NN-GoP} \cite{hu2015improved} improves GMM-GoP by incorporating NN for phoneme prediction and modifying the score function as follows:
\begin{align}
    \Bar{P}(p|F) = \mathbb{E}_F[P^f(p|f)] = \frac{1}{|F|} \sum_{f \in F} P^f(p|f)\\
    s_\text{NN-GoP}(p) = \log \Bar{P}(p|F) - \max_{q \in Q} \log \Bar{P}(q|F)
\end{align}
which is similar to using margin rather than the probability as the uncertainty estimator \cite{kye2022tidal}.
Similarly, \textbf{CALL-GoP} \cite{hu2013new} directly uses the margin as follows:
\begin{align}
    s_\text{CALL-GoP}(p) = \Bar{P}(F|p) - \max_{q \in Q - \{p\}} \Bar{P}(F|p),
\end{align}
based on the acoustic model predictions $P(F|p)$.
Note that if we regard $P(F)$ to be constant, $P(F|p) \propto P(F \cap p) = P(p|F) / P(p)$, which becomes \textbf{DNN-GoP} \cite{hu2015improved}:
\begin{align}
    s_\text{DNN-GoP}(p) = \Bar{P}(p|F) / P(p).
\end{align}


\subsection{Modifying the scoring function}\label{subsec:modify_score}
\cite{kye2022tidal} utilizes \textbf{Entropy} $H$ and \textbf{Margin} $M$ scoring function to measure the data uncertainty:
\begin{align}
    s_\text{H}(p) = -\sum_{q \in Q} \Bar{P}(q|F) \log \Bar{P}(p|F), \\
    s_\text{M}(p) = \Bar{P}(p|F) - \max_{q \in Q - \{p\}} \Bar{P}(q|F).
\end{align}
Even though the above shows the scoring functions formulated with the averaged probability $\Bar{P}$, we can extend the approach to modified probabilities, such as normalized, scaled, or perturbed probabilities in \cref{subsec:modify_score}.


\textbf{MaxLogit} \cite{hendrycks2022scaling} removes the Softmax function to reveal the raw logits for less skewed score distribution:
\begin{equation}
    s_\text{MaxLogit}(p) = \mathbb{E}_F[L^f(p|f)] = \frac{1}{|F|} \sum_{f \in F} L^f(p|f).
\end{equation}
Even though one cannot apply entropy $H$ to unnormalized scores as above, margin $M$ can be still utilized.

% Redesigning

\subsection{Modifying the phoneme predictor}\label{subsec:modify_pred}
We first revisit the approach DNN-GoP \cite{hu2015improved}, which removes the phone bias by dividing with $P(p)$:
\begin{align}
    P_\textbf{DNN-GoP}(p|f) = \frac{e^{L^f(p|f) - \log P(p)}}{ \sum_{q \in Q} e^{L^f(q|f) / T - \log P(q)}},
\end{align}
which can be understood as \textbf{Logit Normalization} with the phoneme probability $\log P(p)$.
Similarly, \textbf{Temperature Scaling} \cite{guo2017calibration} scale the logits with the hyperparameter $T$:
\begin{equation}
    P_\textbf{TS}(p|f) = \frac{e^{L^f(p|f) / T}}{ \sum_{q \in Q} e^{L^f(q|f) / T}},
\end{equation}
where $T$ is obtained by minimizing the negative log loss (NLL) of the validation dataset predictions $P(p|F)$.


\textbf{ODIN} \cite{liang2018enhancing} takes a different approach by perturbing the input speech $f$:
\begin{align}
    \Tilde{f} = f - \epsilon (- \nabla_f \log \max_p P(p|f))\\
    P_\text{ODIN}(p|f) = P(p|\Tilde{f})
\end{align}
where $\epsilon$ is the perturbation magnitude, being added to decrease the final probability $P(p|f)$ of the NN-driven prediction.
\textbf{Mahalanobis \cite{lee2018simple}} removes the need of prediction altogether by measuring the Mahalanobis distance in the latent domain.


==> sections/_4_result.tex <==
% \section{Results} \label{sec:results}
% \input{figures/result}

% \subsection{Pronunciation scoring} \label{ssec:score}
% Scores by severity levels




